TF-Ranking: Scalable TensorFlow Library for Learning-to-Rank

Learning-to-Rank deals with maximizing the utility of a list of examples presented to the user, with items of higher relevance being prioritized. It has several practical applications such as large-scale search, recommender systems, document summarization and question answering. While there is widespread support for classification and regression based learning, support for learning-to-rank in deep learning has been limited. We propose TensorFlow Ranking, the first open source library for solving large-scale ranking problems in a deep learning framework. It is highly configurable and provides easy-to-use APIs to support different scoring mechanisms, loss functions and evaluation metrics in the learning-to-rank setting. Our library is developed on top of TensorFlow and can thus fully leverage the advantages of this platform. For example, it is highly scalable, both in training and in inference, and can be used to learn ranking models over massive amounts of user activity data, which can include heterogeneous dense and sparse features. We empirically demonstrate the effectiveness of our library in learning ranking functions for large-scale search and recommendation applications in Gmail and Google Drive. We also show that ranking models built using our model scale well for distributed training, without significant impact on metrics. The proposed library is available to the open source community, with the hope that it facilitates further academic research and industrial applications in the field of learning-to-rank.

==> lib.tex <==
\section{Implementation} \label{sec:lib}

Our library is based on TensorFlow. Similar to design patterns in TensorFlow, it provides functions and closures for users to construct models and also allows users to build custom functions if needed. 
More specifically, we use the TensorFlow Estimator framework \cite{cheng2017tensorflow} to build ranking models. This framework supports both local and distributed training. The core component of this framework is a \texttt{model\_fn} function that takes features and labels as input and returns loss, prediction, metrics, and training ops, depending on the mode (\texttt{TRAIN, EVAL, PREDICT}). 


The \textttt{tf.Estimator} framework has two main components: (1) An \texttt{input\_fn}, which reads in data from a persistent storage to output Tensors for features and labels, and (2) A \texttt{model\_fn} which processes input features and labels and returns the predictions, loss functions and evaluation metrics, depending on the mode (\texttt{TRAIN, EVAL, PREDICT}). We describe how we implement these two components for learning-to-rank.




\subsection{Input Format}
A ranking problem usually has a context (e.g., a query) and a list of examples. For the sake of simplicity, we assume that all the examples have the same set of features. These features can be sparse or dense. For sparse features, we use embeddings to densify them. 

Our library allows users to specify features (e.g., dense or sparse) using a TensorFlow library such as \texttt{tf.feature\_column}. We allow closures for customized feature transformations and provide utility functions for these transformations.


 The input as represented as a 2-D tensor for each context feature and a 3-D tensor for each candidate feature. Each input feature has a corresponding Feature Column (\texttt{tf.feature\_column}), which denotes whether the feature is dense or sparse, and the type of elements in that tensor. For sparse features, it also specifies a vocabulary and an embedding lookup to convert sparse features to dense features. The embedding layer can be shared between features with the same vocabulary. \\  

        
\textbf{Feature Transformations}. Transform functions are transformations applied to output of  \texttt{input\_fn}. The neural network in scoring function can only take dense tensors as input. The library provides standard functions to transform raw tensors to dense tensors (\texttt{ranking.make\_listwise\_transform\_fn}), and apply shared embeddings over sparse features with the same vocabulary. The user can define a custom \texttt{tfr.feature.make\_transform\_fn} to define any additional feature transformations.


\subsection{Model Building}

\begin{figure*}
\centering
\fbox{
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[width=\linewidth,keepaspectratio]{images/tf_ranking_architecture}

\end{minipage}
}
\fbox{
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[width=\linewidth, keepaspectratio]{images/pseudocode}
\end{minipage}
}
\caption{Building a \texttt{model\_fn} using TensorFlow Ranking library.}
\label{fig:arch}
\end{figure*}

The overall flow of building a \texttt{model\_fn} is shown in Figure~\ref{fig:arch}. There are two important components:
\begin{itemize}
    \item \textbf{Scoring Function}. We focus on single-item scoring functions and multi-item scoring functions~\cite{wang2018groupwise} in this paper. A single-item scoring function takes all context features and all features for a single example as input and outputs a score, as defined in Equation~\ref{eq:pointwise_scoring}. A multi-item scoring function extends this to a group of examples. Conceptually, we slice the tensor for each example list into a number of tensors with shape of \texttt{[batch\_size, group\_size, feature\_size]}, where $\texttt{group\_size} = 1$ for pointwise scoring functions. These group features are combined with context features, and passed to the scoring function to generate scores. After the scoring phase, a voting layer is applied to obtain a tensor with shape \texttt{[batch\_size, list\_size]} for scores, as shown in Figure~\ref{fig:arch} for a mini-batch. The scoring function is a user-specified closure which is passed to the ranking \texttt{model\_fn} builder.
    
    \item \textbf{Ranking Head}. The ranking head structure computes ranking metrics and ranking losses, given scores, labels and optionally example weights. 
    In our library, both score and labels tensors have the same shape \texttt{[batch\_size, list\_size]}, representing \texttt{batch\_size} number of example lists. Ranking head also incorporates example weights, described in Section~\ref{sec:example_weights}, which can be per-example with shape \texttt{[batch\_size, list\_size]} or for the entire list with shape \texttt{[batch\_size]}. Ranking head is available in the library via the factory method \texttt{tfr.head.create\_ranking\_head}.
\end{itemize}














  
  

  




As shown in Figure~\ref{fig:arch}, our library provides factory methods to create metrics and losses. Furthermore, our APIs allow to specify loss functions when creating a ranking head. This enables the user to switch between different loss functions or combine multiple loss functions easily. More importantly, we provide a builder function that takes a scoring function and a ranking head and returns a \texttt{model\_fn} to construct a \texttt{tf.estimator.Estimator}. When \texttt{mode = PREDICT} in \texttt{model\_fn}, the learned scoring function is exported for serving.



==> related_work.tex <==

\section{Related Work}

==> scale.tex <==



